Milky Way Tomography IV: Dissecting Dust

We use SDSS photometry of 73 million stars to simultaneously obtain best-fit main-sequence stellar energy distribution (SED) and amount of dust extinction along the line of sight towards each star. Using a subsample of 23 million stars with 2MASS photometry, whose addition enables more robust results, we show that SDSS photometry alone is sufficient to break degeneracies between intrinsic stellar color and dust amount when the shape of extinction curve is fixed. When using both SDSS and 2MASS photometry, the ratio of the total to selective absorption, $R_V$, can be determined with an uncertainty of about 0.1 for most stars in high-extinction regions. These fits enable detailed studies of the dust properties and its spatial distribution, and of the stellar spatial distribution at low Galactic latitudes. Our results are in good agreement with the extinction normalization given by the Schlegel et al. (1998, SFD) dust maps at high northern Galactic latitudes, but indicate that the SFD extinction map appears to be consistently overestimated by about 20% in the southern sky, in agreement with Schlafly et al. (2010). The constraints on the shape of the dust extinction curve across the SDSS and 2MASS bandpasses support the models by Fitzpatrick (1999) and Cardelli et al. (1989). For the latter, we find an $R_V=3.0\pm0.1$(random) $\pm0.1$(systematic) over most of the high-latitude sky. At low Galactic latitudes (|b|<5), we demonstrate that the SFD map cannot be reliably used to correct for extinction as most stars are embedded in dust, rather than behind it. We introduce a method for efficient selection of candidate red giant stars in the disk, dubbed "dusty parallax relation", which utilizes a correlation between distance and the extinction along the line of sight. We make these best-fit parameters, as well as all the input SDSS and 2MASS data, publicly available in a user-friendly format.

==> figures.tex <==
%%%% Figures for Tomogprahy V %%%%
%% to go back to high resolution figures, remove .png.ps from each file name


\clearpage

%%%%%%%%%%%%%%%%% introduction %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\plotone{Figures/Allsky_SDSS.ps}
\caption{The sky coverage for SDSS Data Release 7, used in this study, in Galactic coordinates. The points show a small random subsample of the full sample of 73 million stars analyzed in this paper. The different colors represent the various data file sets (blue, $\textit{b}>45^{\circ}$; green, $45^{\circ}>\textit{b}>30^{\circ}$; black, the 10 SEGUE strips; yellow, $|\textit{b}|<30^{\circ}$, stars not in SEGUE strips; and red, $\textit{b}<-30^{\circ}$). 
}
\label{Fig:sky}
\end{figure}

\begin{figure}[!t]
\epsscale{0.9}    
\plotone{Figures/PCexamples.ps}
\epsscale{1.0}
\vskip -0.3in    
\caption{The distribution of unresolved SDSS sources with 2MASS detections
in the $\lambda-r$ vs. $r-K$ color-color diagrams, with $\lambda=u, g, i, z, J$ 
and $H$. The source density is shown as color-coded maps, and it increases from 
black to green to red. The two arrows marked PC$_1$ and PC$_2$ in the top left 
panel illustrate the ``principal color'' axes discussed in text and used to 
track the locus shifts due to interstellar dust reddening. The dashed vector 
in each panel shows the reddening vector for $A_r=2$ and standard $R_V=3.1$ 
dust \citep{CCM}.}
\label{Fig:PCex}
\end{figure}


\begin{figure}[!t]
\epsscale{0.9}    
\plotone{Figures/redlawsource.ps}
\epsscale{1.0}
\vskip -0.3in    
\caption{Model predictions for the extinction curve shape as a function 
of $R_V$ for three different models: O'D \citep{ODonnell}, F99 \citep{Fitz99},
and CCM \citep{CCM}, evaluated for stars with three different effective 
temperatures (as listed in the legend, in Kelvin). The left panel shows 
$C_\lambda=A_\lambda/A_r$ for $\lambda=(u,g,r,i,z,J,H,K)$ (top to bottom, 
respectively); the right panel is analogous, except that the ratios
based on colors ($u-g$, $g-r$, $r-i$, $i-z$, $z-J$, $J-H$, and $H-K$) are 
shown. As expected, most of the sensitivity to $R_V$ comes from the blue 
bands ($u$ and $g$).}
\label{Fig:Ed1}
\end{figure}


\begin{figure}[!t]
\epsscale{0.9}    
\plotone{Figures/redlawsourcefits.ps}
\epsscale{1.0}
\vskip -0.3in    
\caption{A comparison of the constraints on the extinction curve shape
(the three plus symbols, with approximate 1$\sigma$ uncertainty limits 
shown as ellipses) and three model predictions (see Figure~\ref{Fig:Ed1} 
for legend; the three crosses along the curves correspond to $R_V$=2.6, 3.1,
and 3.6). The pink symbol corresponds to the Stripe 82 region (southern
Galactic hemisphere), the brown symbol to the northern Galactic hemisphere,
and the blue symbol is the constraint from the Schlafly et al. (2010) analysis.
The blue \citep{Fitz99} and green \citep{CCM} models are in fair agreeement with 
the data, while the red model \cite{ODonnell} predicts unacceptable values of the 
$(A_r-A_i)/(A_i-A_z)$ ratio for all values of $R_V$ (see also 
Figure~\ref{Fig:RvConstraints}).} 
\label{Fig:Ed2}
\end{figure}


\begin{figure}[!t]
\epsscale{0.9}    
\vskip -0.7in    
\plotone{Figures/plotAlambdaRv.ps}
\epsscale{1.0}
\vskip -1.3in    
\caption{Constraints on $R_V$ based on the CCM \citep{CCM} dust reddening
law. Only the SDSS bands, which provide the strongest constraints on $R_V$,
are shown (see the legend). The dashed line shows the overall constraint
on $R_V$ (posterior probability distribution for a flat prior), with 
the best-fit value of $R_V=3.01\pm0.05$.}
\label{Fig:RvConstraints}
\end{figure}



\begin{figure}[!t]
\epsscale{0.9}    
\vskip -0.7in    
\plotone{Figures/plotAlambdaRv_ODonnell.ps}
\epsscale{1.0}
\vskip -1.3in    
\caption{Analogous to Figure~\ref{Fig:RvConstraints}, except that 
\citet{ODonnell} dust reddening law is used. The 
predicted extinction in the $i$ band is inconsistent with 
constraints from other bands.}
\label{Fig:RvOD}
\end{figure}


\begin{figure}[!t]
\epsscale{1.0}
\vskip -0.7in
\plotone{Figures/odccmdiff.ps}
\vskip -0.1in
\caption{The left panel shows the CCM (black, solid line) and the O'Donnell (red, dashed line) 
dust reddening laws as function of wavelength. The right panel displays the fractional difference 
between the two dust extinction models with the SDSS filter transmission regions overlaid (vertical, 
blue, dashed lines). Given the filter transmission regions, the largest integrated difference is 
expected in the $i$ band, which is what we observe.}
\label{Fig:ODCCMdiff}
\end{figure}



\begin{figure}[!t]
\plotone{Figures/rvlin.ps}
\caption{The adopted $A_{\lambda}/A_r$ ratio, shown as a function of 
$R_V$, for $\lambda=(ugrizJHK)$, from top to bottom ($A_r=1$).  The curves are computed
for an F star using the CCM \citep{CCM} dust reddening law.}
\label{Fig:AlambdaRv}
\end{figure}


\begin{figure}[!b]
\epsscale{1.06}        
\hskip -0.5in
\plotone{Figures/panels1.ps}
\epsscale{1.0}        
\vskip -2in
\caption{
An illustration of the constraints on intrinsic stellar colors,
extinction in the $r$ band, $A_r$, and the ratio of total to selective
extinction, $R_V$. In both diagrams, the linearly-spaced 
contours show the main stellar locus as observed at high Galactic
latitudes. The dashed lines mark the median stellar locus from 
\citet{Covey07}. In the left panel, the dot marked ``Obs''
represents a hypothetical observation. Depending on the adopted 
$R_V$, as marked, different combinations of intrinsic stellar 
colors (i.e., the position along the stellar locus) and $A_r$ 
are consistent with the observed $g-r$ and $r-i$ colors. Multiple
solutions are possible even for a fixed value of $R_V$. The
three solutions marked 1-3 correspond to ($R_V$,$A_r$)=
1:(2.2,1.0), 2:(5.0,2.2), and 3:(5.0,6.0). As shown in the right 
panel, these degeneracies are broken if the $i-z$ color is 
also available: the three ($R_V$,$A_r$) combinations have 
different reddened $i-z$ colors which breaks the degeneracy between
the intrinsic stellar color and $A_r$. The degeneracy is broken
because the reddening vectors in the right panel are nearly parallel 
despite very different $R_V$ values.}
\label{Fig:riVSgr}
\end{figure}


%%%%%%%%%%%%%%%%%%% algorithm tests  %%%%%%%%%%%%%%%%% 
\clearpage
\begin{figure}[!t]
\plotone{Figures/aGC_err_m100_a1.5_Dgi.ps}
\caption{A Monte Carlo study of best-fit stellar model errors (parametrized by the 
$g-i$ color) as a function of photometric errors, for a fiducial star with $g-i$=1.95 
and $A_r$=1.5 (the abscissa, $\Delta$$g-i$=true - fit). The photometric errors are generated 
from Gaussian distributions with widths equal to 0.01 mag (top left), 0.02 mag (top right), 
0.04 mag (bottom left) and 0.08 mag (bottom right). The errors in the best-fit
$g-i$ are about twice as large as assumed photometric errors.}
\label{Fig:Dgi}
\end{figure}


\begin{figure}[!t]
\plotone{Figures/aGC_err_m100_a1.5_Dar.ps}
\caption{Analogous to Fig.~\ref{Fig:Dgi}, except that the
errors in the best-fit $A_r$ are shown ($\Delta$$A_r$)=true - fit). 
Note that for large photometric errors (the bottom two panels),
the $A_r$ error distribution becomes bimodal; the additional mode corresponds
to a solution with a bluer star with more reddening.}
\label{Fig:Dar}
\end{figure}


\begin{figure}[!t]
\plotone{Figures/aGC_err_ma_sp_t.ps}
\caption{Analysis of the covariance in the best-fit values for
$A_r$ and $g-i$ using a simulated dataset. The panels show the distributions
of the best-fit values for $A_r$ and $g-i$ for two different fiducial stars 
(left column: a blue star with true $g-i$=0.4; right column: a red star 
with true $g-i$=3.0), and two different extinction values (top panels: 
$A_r=1$; bottom panels: $A_r$=3). Photometric errors in the $ugriz$ bands
are generated using Gaussian distributions with $\sigma$=0.02 
mag (uncorrelated between different bands). Note that the 
$A_r$ vs. $g-i$ covariance is larger for the blue star, and does not
strongly depend on assumed $A_r$.}
\label{Fig:DgiChi2}
\end{figure}
\clearpage


\begin{figure}[!t]
\vskip -0.2in
\epsscale{0.8}
\plotone{Figures/panels1Galfast.ps}
\vskip -1.4in
\caption{Analysis of a {\it Galfast} simulated SDSS-2MASS sample from a SEGUE strip 
($l\sim 110^\circ$ and $|b|<5^\circ$). The $r$ vs. $g-i$ color-magnitude diagrams in the 
top two panels explain why the fraction of giants is much larger than observed at high Galactic 
latitudes. The same simulated sample, defined by {\it observed extincted} magnitude cuts 
$14<r<21$ and $K<14.3$ (Vega)  is shown in both panels. The left panel is constructed using 
{\it un-extincted} magnitudes, and the right panel with ``observed'' magnitudes (note the offset of the 
y axis by 2 mag). The horizontal dashed line in the left panel shows the SDSS saturation limit; 
stars above this line are dominated by red giants (the ``plume'' towards towards $g-i\sim1$). 
The diagonal dashed line shows the magnitude limit for main sequence stars with $K<14.3$ and 
{\it no dust extinction}. The reddening arrow corresponds to $A_r=2$ and $R_V=3.1$ CCM 
extinction curve. The bottom left panel is analogous to the top left panel, except that the 
SDSS-based best-fit values for $g-i$ and $A_r$ are used. The bottom right panel shows the difference between 
the input value of $A_r$ and the best-fit values, as a function of the latter. The dashed line is added to 
guide the eye.  The root-mean-square scatter for the $A_r$ difference (rms for y axis) is 0.33 mag,
and the bias for large $A_r$ is about 15\% (an overestimate of $A_r$ due to color-$A_r$ degeneracy, 
see text). 
}
\label{Fig:mock2}
\end{figure}


\begin{figure}[!t]
\epsscale{0.8}
\vskip -0.2in
\plotone{Figures/mar_rv_SD_new_l110_mock_col.ps}
\vskip -0.3in
\caption{A comparison of six SDSS-2MASS color-color diagrams for data from the SEGUE 
$l\sim 110^\circ$ strip (the top six panels), and for a mock catalog produced with the {\it Galfast} 
code (the bottom six panels). The color-coded contours shows the source counts on a linear 
scale. The two dashed arrows show reddening vectors for $A_r=2$ and $R_V=2$ and 4. The 
locus of circles shows the \citet{Covey07} empirical SED library and illustrates the morphology 
of the same diagrams observed at high Galactic latitudes (and corrected using the SFD map; 
typically $A_r\sim0.1$). The two sets of diagrams are encouragingly similar, with a few detailed 
differences: the observed diagrams have more outliers, and a few diagrams (e.g., $J-K$ vs. $i-z$ 
and $i-z$ vs. $r-i$) imply different reddening vectors than used in simulations ($R_V=3.1$).}
\label{Fig:mock}
\end{figure}



\begin{figure}[!t]
\vskip -0.8in
%\epsscale{0.8}
\epsscale{0.95}
\plotone{Figures/RvHist_clippedChi2.ps}
\vskip -3.0in
\caption{A comparison of the best-fit $R_V$ values for SDSS-2MASS (narrow histogram) and only-SDSS 
(broad histogram) cases, using a simulated {\it Galfast} mock catalog. The input value is fixed to $R_V=3.1$. 
The equivalent Gaussian widths determined from the interquartile range are 0.1 and 1.2, respectively. }
\label{Fig:GalfastRv}
\end{figure}



\begin{figure}[!t]
\vskip -0.8in
\epsscale{0.8}
\plotone{Figures/panelsDPR.ps}
\vskip -1.5in
\caption{The left panel shows the relationship between best-fit $A_r$ and distance computed using 
the SDSS-based best-fit stellar color and a photometric parallax relation appropriate for main sequence stars,
for the same simulated sample as in Figures~\ref{Fig:mock2} and \ref{Fig:mock}. The color-coded
map shows the counts of stars on a linear scale. The dashed lines isolate candidate red giant stars that 
have small distances and large $A_r$. The top right panel is analogous to the top left panel, except 
that the best-fit values correspond to SDSS-2MASS data. The bottom left panel shows the median input
absolute magnitude ($M_r$) for stars in each pixel, color coded according to the legend in the lower
right corner. The ``red giant region'' in the top two panels is dominated by giants ($M_r<3$). 
The bottom right panel shows the difference between true absolute magnitude and an estimate obtained 
from the ``dusty parallax relation'' (see eq.~\ref{eq:DPR}), as a function of the latter. The dashed line has 
is added to guide the eye. The root-mean-square scatter between the two magnitudes 
(rms for y axis) is 1.1 mag.}
\label{Fig:DPR}
\end{figure}

\clearpage



%%%%%%%%%%%%%%%%%%%   analysis of results  %%%%%%%%%%%%%%%%% 

%%% Analysis: introduction ###

\begin{figure}[!t]
\epsscale{0.6}
\vskip -0.3in
\plotone{Figures/p2_hist_NGC_l110_chi2.ps}
\vskip -0.3in
\caption{The distribution of the best-fit $\chi^2_{\mathrm{pdf}}$ ($R_V=3.1$), with differential
distributions in the left two panels, and cumulative distributions in the right two
panels. The top two panels correspond to the north Galactic cap region ($b>45^\circ$)
and the bottom two panels to the SEGUE $l\sim110^\circ$ strip, limited to $|b|<5^\circ$
(a high-extinction region). The solid lines are used for SDSS-only fits, and the dashed 
lines for fits to SDSS-2MASS data. In the two left panels, the top solid line corresponds 
to subsamples of stars with $r<20$, and the bottom solid line to stars with $20<r<21$. 
The top dashed line corresponds to the full SDSS-2MASS sample, and the bottom dashed 
line to subsamples with $K<13.9$  (Vega scale, approximately corresponding to $K$ band 
errors up to 0.05 mag). The solid lines in the right panels correspond to the full SDSS sample, 
and the short-dashed lines to the full SDSS-2MASS sample. The dot-dashed and long-dashed
lines correspond to $\chi^2_{\mathrm{pdf}}$ distributions with 2 and 5 degrees of freedom. The 
long-dashed line in the top left panel corresponds to the $\chi^2_{\mathrm{pdf}}$ distribution 
with 5 degrees of freedom for the full SDSS-2MASS sample.
}
\label{Fig:Chi2Slices110}
\end{figure}



\begin{figure}[!t]
\epsscale{0.9}
\phantom{x}
\vskip -3.0in
\plotone{Figures/panels_LambertNGP.ps}
\vskip -1.5in
\caption{Analysis of the best-fit results for $A_r$ in the low-extinction region with $b>30^\circ$.
The top left panel shows the median $A_r$ in 0.6 deg$^2$ pixels in Lambert projection.
The values are linearly color-coded according to the legend.
Stars with $15<r<18$ and $\chi^2_{\mathrm{pdf}}<2$ from only-SDSS sample with fixed $R_V$
are used for the plot. The median difference between $A_r$ and the values given by the SFD map
are shown in the top right panel. Note the striping reminiscent of the SDSS scanning pattern. 
The bottom left panel shows the median difference between observed and best-fit model magnitudes
in the $i$ band. The bottom right panel is analogous to the top right panel, except that only the
subset of stars also detected by 2MASS ($K<14$) and with full SDSS-2MASS fits (fixed $R_V$) 
are used. Note the much better agreement with the SFD values than in the top right panel. For
more details, please see \S\ref{sec:ngp}.}
\label{panelsLambertNGP}
\end{figure}



\begin{figure}[!t]
\epsscale{0.8}
\vskip -0.7in
\plotone{Figures/panels_SDSSonly_5deg.ps}
\vskip -0.3in
\caption{The color-coded maps show the best-fit $A_r$ based on SDSS 
data for the ten analyzed SEGUE stripes. Each stripe is limited to the range 
of $|b|<5^\circ$. A fixed $R_V=3.1$ is assumed. 
The legend above each panel shows the color scale, and each 12$\times$12 
arcmin$^2$ pixel shows the median $A_r$. For each stripe, three 
distance ranges are shown: 0.3-0.6 kpc (left), 1-1.5 kpc (middle) 
and 2-2.5 kpc (right). It is assumed that all stars are on 
main sequence when estimating distances. Only stars with best-fit 
$\chi^2_{pdf}<2$ and outside the red giant region (selected here by 
$A_r<1.5+1.5\,D_{\rm kpc}$) are used for the plot. The top right panel 
shows the sky coverage of the full analyzed dataset.}
\label{Fig:ArSDSSdSlicesAll}
\end{figure}



\begin{figure}[!t]
\vskip -1.8in
\epsscale{0.8}
\plotone{Figures/DAcounts_onlySDSS.ps}
\vskip -0.7in
\caption{The counts of stars in the only-SDSS case best-fit $A_r$ vs. best-fit main 
sequence distance diagram for four SEGUE strips (top left: $l=70^\circ$, top right: $l=110^\circ$, 
bottom left: $l=150^\circ$, bottom right: $l=187^\circ$; for all panels $|b|<5^\circ$). 
Only stars with $\chi^2_{\mathrm{pdf}}<2$, $r<19$ and error in the $u$ band below 0.05 mag are used. Counts are 
normalized to the maximum value and color coded on the same linear scale, from blue (low) to 
red (high). The two dashed lines mark a region dominated by red giant stars (the top left corner).}
\label{Fig:DAcounts_onlySDSS}
\end{figure}



\begin{figure}[!t]
\vskip -1.8in
\epsscale{0.8}
\plotone{Figures/DAcounts_SDSS2MASS.ps}
\vskip -0.7in
\caption{
Analogous to Figure~\ref{Fig:DAcounts_onlySDSS}, except for best-fits based on SDSS-2MASS sample
(only stars with $\chi^2_{\mathrm{pdf}}<2$ and $K<15$ on Vega scale are used). Note the larger 
fraction of red giant stars in the top left corner, and a smaller distance limit, compared 
to Figure~\ref{Fig:DAcounts_onlySDSS} and that the fraction of giants decreases with 
Galactic longitude.}
\label{Fig:DAcounts_SDSS2MASS}
\end{figure}





%%%%%%   l=110 strip in detail:


\begin{figure}[!t]
\epsscale{0.8}
\vskip -0.2in
\plotone{Figures/SEGUEl110_dataVSfixedRv.ps}
\vskip -0.3in
\caption{A comparison of six SDSS-2MASS color-color diagrams using data from the SEGUE 
$l\sim 110^\circ$ strip (the top six panels; same as the top six panels in Figure~\ref{Fig:mock}, except
that here only stars with $\chi^2_{\mathrm{pdf}}<2$ are used), and the best-fit model colors based on  
SDSS-2MASS dataset (the bottom six panels, in the same order). The thick lines show the 
\citet{Covey07} empirical SED library and illustrate the 
morphology of the same diagrams observed at high Galactic latitudes. The two sets of diagrams are 
encouragingly similar: fits to intrinsic stellar SED and dust extinction on per star basis are
capable of reproducing the morphology of observed diagrams in highly dust-extincted regions.}
\label{Fig:CMD_SEGUEl110_dataVSfixedRv}
\end{figure}


\begin{figure}[!t]
\epsscale{1.0}
\vskip -0.7in
\plotone{Figures/compareArGI_onlySDSSvsSDSS2MASS.ps}
\vskip -0.1in
\caption{A comparison of the best-fit $g-i$ (left panel) and $A_r$ (right panel)
values obtained with a fixed $R_V=3.1$ for SDSS-2MASS sample from the SEGUE 
$l\sim110^\circ$ stripe, using two different fitting methods. 
The abscissae show the best-fit values obtained using only-SDSS dataset (four fitted
colors), and the ordinates correspond to the residuals of the SDSS-2MASS (seven fitted colors) 
minus the only-SDSS datasets. The number density of stars increases linearly from black to blue 
to red. The dashed lines are added to guide the eye. }
\label{Fig:compareArGI_onlySDSSvsSDSS2MASS}
\end{figure}


\begin{figure}[!t]
\epsscale{0.6}
\vskip -0.3in
\plotone{Figures/sdss_2mass_lvb_b30_l110_SD.ps}
\vskip -0.3in
\caption{Analysis of the differences in the best-fit $A_r$ between fits based on 
SDSS-2MASS dataset (first panel from the left) and those based on only-SDSS data
(second panel). Only stars with best-fit $\chi^2_{pdf}<2$, $r<20$ and main-sequence
distance $0.5-1$ kpc are used for the plot. The top legend shows the coloring code for 
these two panels, and each 6$\times$6 arcmin$^2$ pixel shows the median $A_r$ for stars with 
$\chi^2_{\mathrm{pdf}}<2$. The third panel shows the median difference between the two best-fit 
$A_r$ values (the second panel minus the first panel), with the color coding using the same 
palette, {\it except that the limits are $\pm0.1$ mag}. The fourth panel shows the median 
difference in $A_r$ (i.e., the third panel) for 0.2$^\circ$ wide bins of Galactic latitude.}
\label{Fig:ArSDSSvsSDSS2MASS}
\end{figure}
 


\begin{figure}[!t]
\epsscale{0.55}
\vskip -0.5in
\plotone{Figures/sdss_lvb_b30_l110_dist.ps}
\epsscale{1.0}
\vskip -0.5in
\caption{The color-coded maps show the best-fit $A_r$ based on only-SDSS 
dataset for the SEGUE $l\sim 110^\circ$ strip. The legend shows the color scale, 
and each 12x12 arcmin$^2$ pixel shows the median $A_r$. The three panels correspond
to main-sequence distance range: $0.3-0.6$ kpc (left), $1-1.5$ kpc (middle) and 
$2-2.5$ kpc (right). Only stars with best-fit $\chi^2_{pdf}<2$ and outside the red giant
region (selected here by $A_r<1.5+1.5\,D_{\rm kpc}$) are used for the plot.}
\label{Fig:ArSDSSdistSlicesSEGUE110}
\end{figure}


\begin{figure}[!t]
\epsscale{0.8}
\vskip -0.9in
\plotone{Figures/sdss_2mass_lvb_b10_l110_dbins.ps}
\vskip -0.5in
\caption{Analogous to Figure~\ref{Fig:ArSDSSdistSlicesSEGUE110}, 
except using the SDSS-2MASS dataset and different distance slices (left to 
right: $0.1-0.5$ kpc, $0.5-0.7$ kpc, $0.7-0.9$ kpc, $0.9-1.1$ kpc). Note the
abrupt increase in $A_r$ for stars towards $b\sim+2^\circ$ that are more distant than 0.9 kpc.}
\label{Fig:ArSDSSdSlices110zi}
\end{figure}



\begin{figure}[!t]
\epsscale{0.6}
\vskip -0.2in
\plotone{Figures/sdss_lvb_b30_l110_SFD.ps}
\epsscale{1.0}
\vskip -0.3in
\caption{Analysis of the differences between best-fit $A_r$ values (left 
panel, based on only-SDSS data; SDSS-2MASS version looks similar) and 
the SFD values (second panel) for stars with $\chi^2_{pdf}<2$ and main-sequence
distance in the range $0.8-1.2$ kpc. The third panel shows the difference of the two 
$A_r$ values (the second panel minus the first panel). Each 6$\times$6 arcmin$^2$ pixel 
in the first three panels is color coded according to the top legend. The fourth panel 
shows the median best-fit $A_r$ (blue line) and the median SFD value (red line) for 
0.2$^\circ$ wide bins of Galactic latitude. If the SFD maps are correct, then the dust 
structures discernible in the two right panels at $b\sim0^\circ$ and $b\sim+2^\circ$ 
must be more distant than $\sim$1 kpc. This conclusion is independently confirmed
for the latter dust cloud in Figure~\ref{Fig:ArSDSSdSlices110zi}.}
\label{Fig:ArSDSScompSFD}
\end{figure}



\clearpage
\begin{figure}[!t]
\epsscale{0.75}
\vskip -0.1in
\hskip 0.0in
\plotone{Figures/Cpanels_110.ps}
\vskip -0.3in
\caption{The bottom four panels show the $|b|<5^\circ$ subregion 
of the panels shown in Fig.~\ref{Fig:ArSDSScompSFD}. The top three
panels show the mid-IR (left), CO (middle) and radio continuum (right)
maps on approximately the same scale (obtained using ``The Milky Way 
Explorer'' by Kevin Jardine). The few small irregular white regions in the bottom three
maps do not contain any stars with good photometry. Assuming that the SFD map is 
not grossly incorrect, the dust extinction determined here implies that most of the molecular 
cloud structures seen in the top middle panel must be more distant than $\sim$1 kpc.}
\label{Fig:KeiraL110}
\end{figure}
% http://galaxymap.org/drupal/node/127




%%%% floating Rv case %%%%%%%

\begin{figure}[!t]
\epsscale{1.0}
\vskip -0.7in
\plotone{Figures/compareArGI_freeVSfixedRv.ps}
\vskip -0.1in
\caption{A comparison of the best-fit $g-i$ (left panel) and $A_r$ (right panel)
values for two different treatments of $R_V$, for stars in the $l=110^\circ$ SEGUE strip
(using SDSS-2MASS data). Only stars with best-fit $\chi^2_{pdf}<2$, $r<20$ and
$K<13.9$ (Vega) are used for the plot. The abscissae show the best-fit values obtained for a fixed 
$R_V=3.1$ and the ordinates correspond to the residuals of the differences in the best-fit values 
when $R_V$ is treated as a free-fitting parameter (``free $R_V$'' $-$ ``$R_V$=3.1''). The number density of 
stars increases from black to blue to red. The dashed lines are added to guide the eye. }
\label{Fig:compareArGI_freeVSfixedRv}
\end{figure}


\begin{figure}[!t]
\vskip -1.8in
\epsscale{0.8}
\plotone{Figures/DAcounts_SDSS2MASS_freeRv.ps}
\vskip -0.7in
\caption{The $A_r$ map analogous to Figure~\ref{Fig:DAcounts_SDSS2MASS}, except that $R_V$ is
treated as a free parameter. Only stars with $|b|<5^\circ$, 
$\chi^2_{\mathrm{pdf}}<2$, $r<19$, and $K<15$ (on Vega scale) are used. 
}
\label{Fig:DAcounts_SDSS2MASS_freeRv}
\end{figure}


\begin{figure}[!t]
\epsscale{1.0}
\vskip -0.7in
\plotone{Figures/frv_SED_nw.ps}
\vskip -0.0in
\caption{A comparison of three different types of best-fit
SEDs: using only SDSS data with fixed $R_V=3.1$ (blue
line), and using joint SDSS-2MASS dataset with fixed $R_V$ (green 
line) and with free $R_V$ (red line).  As demonstrated by the 
similarity of best-fit lines, the differences in best-fit parameters,
listed in each panel, are due to degeneracies between intrinsic
stellar color, amount of dust and $R_V$. The shown cases
correspond to blue and red stars (top row vs. bottom row), and
small and large $A_r$ (left column vs. right column).}
\label{Fig:FRVSED}
\end{figure}


\begin{figure}[!t]
\vskip -1.8in
\epsscale{0.8}
\plotone{Figures/DAmedRv_SDSS2MASS_freeRv.ps}
\vskip -0.7in
\caption{Similar to Figure~\ref{Fig:DAcounts_SDSS2MASS}, except that $R_V$ is
treated as a free parameter, and the color-coded map shows the median value of
$R_V$ (ranging from blue for $R_V=1.5$ to red for $R_V=4.5$, green corresponds 
to $R_V=3$; see the legend in the bottom right panel). Only stars with $|b|<5^\circ$, 
$\chi^2_{\mathrm{pdf}}<2$, $r<19$, and $K<15$ (on Vega scale) are used. 
Note that red giant stars (top left corner) have consistently larger values of $R_V$, and
that consistently $R_V<3$ when $A_r < 1$ for main sequence stars. In other
regions in this diagram where $R_V$ is determined robustly, $R_V=3.1$ cannot be 
ruled out in any of the ten SEGUE stripes at a precision level of $\sim0.1-0.2$.  
}
\label{Fig:DAmedRv_SDSS2MASS_freeRv}
\end{figure}


\begin{figure}[!t]
\vskip -0.8in
%\epsscale{0.8}
\epsscale{0.95}
\plotone{Figures/RvHist_SEGUE_l70_l110.ps}
\vskip -3.0in
\caption{A comparison of the best-fit $R_V$ values for SDSS-2MASS free-$R_V$ case
and stars with distances in the 1.0-2.5 kpc range and $A_r>2.5$, selected from 
$l=70^\circ$ (red, left histogram) and $l=110^\circ$ (blue, right histogram) stripes 
(other selection criteria are the same as for stars plotted in 
Figure~\ref{Fig:DAmedRv_SDSS2MASS_freeRv}).}
\label{Fig:RvHist_SEGUE_l110}
\end{figure}


\begin{figure}[!t]
\epsscale{0.7}
\vskip -0.3in
\plotone{Figures/sd2m_frv_lvb_b30_l110_dist.ps}
\epsscale{1.0}
\vskip -0.3in
\caption{The first three panels show the median $R_V$ obtained using SDSS-2MASS 
sample for the SEGUE $l=110^\circ$ strip, and for distance range $0.5-0.7$ kpc (first), 
$0.7-0.9$ kpc (second), and $0.9-1.1$ kpc (third). Only stars outside the 
``red giant'' region, see Figure~\ref{Fig:DAcounts_SDSS2MASS}, and with 
$\chi^2_{pdf}<2$, $r<21$ and $K<14.3$ (Vega) are used for the plot. The pixel size 
is 6$\times$6 arcmin$^2$, and the $R_V$ coloring scheme is shown at the top. 
The fourth panel shows for reference the best-fit $A_r$, for the distance slice $0.9-1.1$ kpc.
Note that $R_V$ is not reliable for $A_r<2$ (black and blue regions in the fourth panel).}
\label{Fig:sd2m_rvmap}
\end{figure}



\begin{figure}[!t]
\epsscale{0.6}
\vskip -0.35in
\plotone{Figures/sdss_lvb_b10_l110_dbins_dif_0_500.ps}
\epsscale{1.0}
\vskip -0.4in
\caption{Illustration of the three-dimensional dust distribution for SEGUE stripe $l\sim110^\circ$
at mean distances of 1.0, 1.5, 2.0 and 2.5 kpc, using only-SDSS sample and fixed-$R_V$ fits.
Unlike other figures that show the median $A_r$ {\it along the line of sight}, this figure shows the 
{\it differences} in the median $A_r$ (per 12$\times$12 arcmin$^2$ pixel) for samples at distances 
between the quoted distance and limiting distances 0.5 kpc larger and smaller than the mean distance 
(e.g., the first panel shows the difference between the median $A_r$ for 0.5-1.0 kpc and 1.0-1.5 kpc 
subsamples). It is easily discernible that the dust structures observed at $b\sim2^\circ$ and 
$b\sim13^\circ$ are confined to 1-1.5 kpc distance range, while the structure seen at $-3^\circ<b<0^\circ$ 
is due to dust at a distance of $\sim2.5$ kpc (an analogous panel for a mean distance of 3.0 kpc 
shows that this structure is mostly confined to smaller distances). Note that the linear extent 
perpendicular to the line of sight of a given angular size is 2.5 times larger in the last than in 
the first panel.}
\label{Fig:sd2m_diffArDslices}
\end{figure}



\clearpage

\begin{figure}[!t]
\epsscale{0.8}
\vskip -0.5in
\plotone{Figures/panelsDxyAr.ps}  
\vskip -0.7in
\caption{The median best-fit $A_r$ (extinction along the line of sight) is shown as 
a function of distance from the Galactic plane, $Z$, and distance along the plane, 
$D_{xy}$, for 10 SEGUE stripes (this is {\bf not} a cross-section of three-dimensional
dust distribution!). The best-fit $A_r$ are based on the SDSS-2MASS dataset and 
fixed-$R_V$ fitting case, for stars with $\chi^2_{pdf}<2$ and $K<15$ (Vega).
Each pixel is 50$\times$50 pc$^2$ and subtends 2.5 deg wide stripe in the perpendicular 
(longitude) direction. The color scheme increases linearly from blue to red with a varying 
maximum value: 5 for the first three panels, 4 for the next three, and 3 for the last four panels.}
\label{Fig:ZDcutArPanels}
\end{figure}


\begin{figure}[!t]
\epsscale{0.8}
\vskip -0.5in
\plotone{Figures/panelsDxyCounts.ps}
\vskip -0.7in
\caption{The local volume number density of stars is shown as a function of 
distance from the Galactic plane, $Z$, and distance along the plane, $D_{xy}$,
for the same samples as shown in Figure~\ref{Fig:ZDcutArPanels}. The color scheme 
shows the counts on log scale with the same arbitrary normalization for all stripes. 
The fall-off of the stellar volume  number density at distances beyond $\sim$1 kpc 
is due to the stellar color-dependent sample distance limit and does not reflect the 
disk structure. Note the variation of counts with Galactic longitude (the top four
panels are closer to the Galactic center and contain more stars per unit volume).}
\label{Fig:ZDcutRhoPanels}
\end{figure}


